Arrow Contraction and Expansion in Tropical Diagrams

Arrow contraction applied to a tropical diagram of probability spaces is a modification of the diagram, replacing one of the morphisms by an isomorphims, while preserving other parts of the diagram. It is related to the rate regions introduced by Ahlswede and K\"orner. In a companion article we use arrow contraction to derive information about the shape of the entropic cone. Arrow expansion is the inverse operation to the arrow contraction.

==> defs.tex <==
\makeatletter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Letters
\let\tmp=\phi \let\phi=\varphi \let\varphi=\tmp
\let\tmp=\epsilon \let\epsilon=\varepsilon \let\varepsilon=\tmp

\let\emptyset=\varnothing
\def\i{{\bm\imath}}
\def\j{{\bm\jmath}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arrows
\newcommand{\into}[1][]{\stackrel{#1}{\hookrightarrow}}
\renewcommand{\to}[1][]{\stackrel{#1}{\rightarrow}}
\newcommand{\too}[1][]{\stackrel{#1}{\longrightarrow}}
\newcommand{\ot}[1][]{\stackrel{#1}{\leftarrow}}
\newcommand{\oot}[1][]{\stackrel{#1}{\longleftarrow}}
\newcommand{\oto}[1][]{\stackrel{#1}{\leftrightarrow}}
\newcommand{\ootoo}[1][]{\stackrel{#1}{\longleftrightarrow}}

% Binary operators
% Definition of \indep is bad
%\def\indep{\,\makebox[0cm][l]{$\bot$}\mkern2mu\bot\,}
\def\indep{\,\makebox[0cm][l]{$\bot$}\,\bot\,}
\def\rel{|\mkern-2.5mu\raisebox{-0.57ex}{\rule{0.3em}{0.15ex}}}
% Brackets
\def\lc{\left\lceil}
\def\rc{\right\rceil}
\def\lf{\left\lfloor}
\def\rf{\right\rfloor}
\def\<{\left\langle}
\def\>{\right\rangle}

\def\size#1{[\mkern-5mu[#1]\mkern-5mu]}

\def\coords(#1;#2;#3;#4){
  \left(
  \begin{array}{c}
    #1\\#2\\#3\\#4
  \end{array}
  \right)
}

% Decorations
\newcommand{\un}[2][5mu]{\underline{#2\mkern-#1}\mkern#1} 
\newcommand{\polar}{\stackrel{\circ}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math Operators
\let\dmo=\DeclareMathOperator
\dmo\dist{\dbf}
\dmo\dista{\deltabf}
\dmo\disth{\deltabf}
\dmo\distha{\hat\deltabf}

\dmo\lin{\Lsf}
\dmo\qlin{\Qsf\Lsf}

\dmo\d@tmp{\drm\mkern-3mu}\let\d=\d@tmp

\dmo\ent{\mathsf{Ent}}
\dmo\prob{\mathbf{Prob}}\let\Prob=\prob
\dmo\Set{\mathbf{Set}}
\dmo\Gr{\mathbf{Gr}}
\dmo\kd{\mathrm{kd}}
\dmo\ikd{\mathbf{k}}
\dmo\aikd{\bm\kappa}
\dmo\Aut{\mathrm{Aut}}
\dmo\stab{\mathrm{Stab}}
\dmo\unif{\mathsf{unif}}
\dmo\lift{\mathsf{Lift}}

\dmo\mix{\Mcal\mkern-2mu\mathit{ix}}
\dmo\emp{\qbf}

\dmo\aep{\mathbf{aep}}

\dmo\smc{\Gamma_{\mathrm{sm}}}
\dmo\ec{\Gamma}
\dmo\abc{\Gamma_{\mathrm{ab}}}

\dmo\ing{\mathsf{ing}}
\dmo\spc{\mathsf{spc}}
\dmo\SH{\mathsf{SH}}

\dmo\O@{\Ocal}\let\O=\O@
\dmo\o@{\scalebox{0.65}{\Ocal}}\let\o=\o@
\dmo\mi{\mathsf{MI}}
\dmo\id{\mathrm{id}}
\dmo\p{\Pbb}%\raisebox{-0.46ex}{\scalebox{0.95}{\Pbb}}}}

\def\smallboldnum#1{{\scriptstyle\mathbf{#1}}}
\def\1{\smallboldnum1}
\def\2{\smallboldnum2}
\def\3{\smallboldnum3}
\def\4{\smallboldnum4}


\skipthis{
\dmo\Set{\mathbf{Set}}
\dmo\Interior{\mathrm{Interior}}
\dmo\d@{\drm\mkern-3mu}\let\d=\d@
\dmo\SH{\mathsf{SH}}
\dmo\sh{\mathsf{sh}}
\dmo\ING{\mathsf{ING}}
\dmo\closure{\mathrm{Closure}}
\dmo\cone{\mathrm{Cone}}
%\def\Mor{\operatorname{Mor}}
%\def\convconend{\mathrm{\Kbf}_{k,l}}
%\def\haus{\operatorname{\mathrm{d}_{h}}}
%\def\distaa{\operatorname{\hatt{\bm\delta}}}
%\def\D{\operatorname{\Dsf}}
%\def\ad{\operatorname{\mathbf{ad}}}
%\def\cs{\operatorname{\Csf\Ssf}}\let\CS=\cs
%\def\ext{\operatorname{\Esf\xsf\tsf}}
%\def\EXT{\operatorname{\Esf\Xsf\Tsf}}
%\def\aep{\operatorname{\mathbf{aep}}}
%\def\IO{\operatorname{\mathrm{IO}}}\let\io=\IO
%\def\Ext{\operatorname{\mathrm{Ext}}}
%\def\Hom{\operatorname{\mathrm{Hom}}}
%\def\closure{\operatorname{\mathrm{Closure}}}
%\def\supp{\operatorname{\mathrm{supp}}}
%\def\defect{\operatorname{\mathrm{Defect}}}
%\def\dia{{\bm\Diamond}}
%\def\emptyconfig{\mkern3mu\raisebox{0.2ex}{\ensuremath{\bm/}}\mkern-13mu\Ocal}
%\def\emptycat{\bm{\emptyset}}
%\def\res{\Gammabf^{\circ}}
%\def\sres{\bar\Gammabf}
%\def\c#1{(\!#1\!)}
%\def\sep{\,||\,}

}

\newcommand{\aeq}[1][\aikd]{\stackrel{#1}{=}}
\newcommand{\bernoulli}[1]{\overrightarrow{#1}}


\makeatother


==> style.tex <==
\usepackage{environ}
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Math letters
\def\mkmathletter#1#2{%
    \expandafter\gdef\csname#1#2\endcsname%
           {\ensuremath{\csname math#2\endcsname{#1}}}%
}
\def\mkmathletters#1{
\mkmathletter{A}{#1}
\mkmathletter{B}{#1}
\mkmathletter{C}{#1}
\mkmathletter{D}{#1}
\mkmathletter{E}{#1}
\mkmathletter{F}{#1}
\mkmathletter{G}{#1}
\mkmathletter{H}{#1}
\mkmathletter{I}{#1}
\mkmathletter{J}{#1}
\mkmathletter{K}{#1}
\mkmathletter{L}{#1}
\mkmathletter{M}{#1}
\mkmathletter{N}{#1}
\mkmathletter{O}{#1}
\mkmathletter{P}{#1}
\mkmathletter{Q}{#1}
\mkmathletter{R}{#1}
\mkmathletter{S}{#1}
\mkmathletter{T}{#1}
\mkmathletter{U}{#1}
\mkmathletter{V}{#1}
\mkmathletter{W}{#1}
\mkmathletter{X}{#1}
\mkmathletter{Y}{#1}
\mkmathletter{Z}{#1}
\mkmathletter{a}{#1}
\mkmathletter{b}{#1}
\mkmathletter{c}{#1}
\mkmathletter{d}{#1}
\mkmathletter{e}{#1}
\mkmathletter{f}{#1}
\mkmathletter{g}{#1}
\mkmathletter{h}{#1}
\mkmathletter{i}{#1}
\mkmathletter{j}{#1}
\mkmathletter{k}{#1}
\mkmathletter{l}{#1}
\mkmathletter{m}{#1}
\mkmathletter{n}{#1}
\mkmathletter{o}{#1}
\mkmathletter{p}{#1}
\mkmathletter{q}{#1}
\mkmathletter{r}{#1}
\mkmathletter{s}{#1}
\mkmathletter{t}{#1}
\mkmathletter{u}{#1}
\mkmathletter{v}{#1}
\mkmathletter{w}{#1}
\mkmathletter{x}{#1}
\mkmathletter{y}{#1}
\mkmathletter{z}{#1}
}
\mkmathletters{frak}
\mkmathletters{bb}
\mkmathletters{cal}
\mkmathletters{bf}
\mkmathletters{rm}
\mkmathletters{sc}
\mkmathletters{sf}
\def\alphabf{\ensuremath{\bm\alpha}}
\def\betabf{\ensuremath{\bm\beta}}
\def\gammabf{\ensuremath{\bm\gamma}}
\def\deltabf{\ensuremath{\bm\delta}}
\def\epsilonbf{\ensuremath{\bm\epsilon}}
\def\zetabf{\ensuremath{\bm\zeta}}
\def\etabf{\ensuremath{\bm\eta}}
\def\thetabf{\ensuremath{\bm\theta}}
\def\jotabf{\ensuremath{\bm\jota}}
\def\kappabf{\ensuremath{\bm\kappa}}
\def\lambdabf{\ensuremath{\bm\lambda}}
\def\mubf{\ensuremath{\bm\mu}}
\def\nubf{\ensuremath{\bm\nu}}
\def\xibf{\ensuremath{\bm\xi}}
\def\pibf{\ensuremath{\bm\pi}}
\def\omikronbf{\ensuremath{\bm\omikron}}
\def\rhobf{\ensuremath{\bm\rho}}
\def\sigmabf{\ensuremath{\bm\sigma}}
\def\taubf{\ensuremath{\bm\tau}}
\def\upsilonbf{\ensuremath{\bm\upsilon}}
\def\phibf{\ensuremath{\bm\phi\phi}}
\def\chibf{\ensuremath{\bm\chi}}
\def\psibf{\ensuremath{\bm\psi}}
\def\omegabf{\ensuremath{\bm\omega}}

\def\Alphabf{\ensuremath{\bm\Alpha}}
\def\Betabf{\ensuremath{\bm\Beta}}
\def\Gammabf{\ensuremath{\bm\Gamma}}
\def\Deltabf{\ensuremath{\bm\Delta}}
\def\Epsilonbf{\ensuremath{\bm\Epsilon}}
\def\Zetabf{\ensuremath{\bm\Zeta}}
\def\Etabf{\ensuremath{\bm\Eta}}
\def\Thetabf{\ensuremath{\bm\Theta}}
\def\Jotabf{\ensuremath{\bm\Jota}}
\def\Kappabf{\ensuremath{\bm\Kappa}}
\def\Lambdabf{\ensuremath{\bm\Lambda}}
\def\Mubf{\ensuremath{\bm\Mu}}
\def\Nubf{\ensuremath{\bm\Nu}}
\def\Xibf{\ensuremath{\bm\Xi}}
\def\Pibf{\ensuremath{\bm\Pi}}
\def\Omikronbf{\ensuremath{\bm\Omikron}}
\def\Rhobf{\ensuremath{\bm\Rho}}
\def\Sigmabf{\ensuremath{\bm\Sigma}}
\def\Taubf{\ensuremath{\bm\Tau}}
\def\Upsilonbf{\ensuremath{\bm\Upsilon}}
\def\Phibf{\ensuremath{\bm\phi\Phi}}
\def\Chibf{\ensuremath{\bm\Chi}}
\def\Psibf{\ensuremath{\bm\Psi}}
\def\Omegabf{\ensuremath{\bm\Omega}}
%% Math Letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% remark
\setlength{\marginparsep}{2mm}
\setlength{\marginparwidth}{10mm}
\newcounter{remarkcounter}\setcounter{remarkcounter}{0}
\def\printremarkcounter{\raisebox{1ex}{%
    \normalfont%
    \footnotesize%
    (\hspace{-0.1em}\alph{remarkcounter}\hspace{-0.1em})}%
}
\def\remark#1{%
  \stepcounter{remarkcounter}%
  \unskip\nopagebreak\printremarkcounter%
  \marginpar{%
    \renewcommand{\baselinestretch}{0.9}%
    \begin{flushleft}
      \makebox[0mm][r]{\printremarkcounter}%
      \small#1
    \end{flushleft}%
  }%
}

\newcommand{\skipthis}[2][]{\relax}
\newcommand{\skipthiss}[2][]{x\relax.}
\let\comment=\skipthis

\long\def\coloredtext#1#2{%
  \begingroup%
    \color{#1}%
    #2%
  \endgroup%
}

\long\def\red#1{\coloredtext{red}{#1}}
\long\def\green#1{\coloredtext{green}{#1}}
\long\def\blue#1{\coloredtext{blue}{#1}}

\long\def\skippar#1\par{\relax\par}
\long\def\justpar#1\par{#1\par}
\newcommand{\justins}[2][]{#2}
\newcommand{\justrm}[2][]{#1}

% \specialpar{color} paragraph \par
% presymbol is put on the left margin at the first line
% prehook could be something like \noindent
\long\def\specialpar#1#2\par{%
  \unskip%
  \rule{0mm}{1ex}\par%
  \coloredtext{#1}{\unskip#2}%
  \par%
}

\def\csletsecond#1#2{%
  \expandafter\let\expandafter#1\csname#2\endcsname}

\def\cslet#1#2{%
  \expandafter\csletsecond\csname#1\endcsname{#2}}

\def\lgdef{\long\global\def}

%\getoption{prefix}{optionname}{defaultvalue}{optionsstring}

\newcommand{\getoption}[4]{%
  \def\get@option##1#2=##2,##3ENDOFTHEARGS{%
    \expandafter\gdef\csname#1#2\endcsname{##2}}%
  \get@option#4,#2=#3,ENDOFTHEARGS}

% \setcolors[rmcolor=cyan,
%            commentcolor=purple,
%            inscolor=blue,
%            commentsymbol=$\bullet$,
%            rmsymbol=$\bullet$,
%            inssymbol=$\bullet$,
%           {jim}

\newcommand{\setcolors}[2][]{%
  \getoption{#2}{rmcolor}{green}{#1}%
  \getoption{#2}{inscolor}{blue}{#1}%
  \getoption{#2}{commentcolor}{red}{#1}%
  \getoption{#2}{commentsymbol}{off}{#1}%
  \getoption{#2}{rmsymbol}{off}{#1}%
  \getoption{#2}{inssymbol}{off}{#1}%
  %
  \expandafter\lgdef\csname#2@par\endcsname{%
    \specialpar{\csname#2commentcolor\endcsname}%
    \noindent\rule{0mm}{1ex}%
    \ifthenelse{\not\equal{\csname#2commentsymbol\endcsname}{off}}{%
    \marginpar{\center\textcolor{\csname#2commentcolor\endcsname}{%
               \csname#2commentsymbol\endcsname}}}{\relax}%           
  }%
  \expandafter\lgdef\csname#2@inspar\endcsname{%    
    \specialpar{\csname#2inscolor\endcsname}%
    \rule{0mm}{1ex}%
    \ifthenelse{\not\equal{\csname#2inssymbol\endcsname}{off}}{%
    \marginpar{\center\textcolor{\csname#2inscolor\endcsname}{%
               \csname#2inssymbol\endcsname}}}{\relax}%
  }%
  \expandafter\lgdef\csname#2@rmpar\endcsname{%
    \specialpar{\csname#2rmcolor\endcsname}%
    \rule{0mm}{1ex}%
    \ifthenelse{\not\equal{\csname#2rmsymbol\endcsname}{off}}{%
    \marginpar{\center\textcolor{\csname#2rmcolor\endcsname}{%
               \csname#2rmsymbol\endcsname}}}{\relax}%
  }%
  \expandafter\def\csname#2@com\endcsname{\relax}
  \expandafter\renewcommand\csname#2@com\endcsname[1]{%
    \rule{0mm}{1ex}%
    \ifthenelse{\not\equal{\csname#2commentsymbol\endcsname}{off}}{%
    \marginpar{\center\textcolor{\csname#2commentcolor\endcsname}{%
               \csname#2commentsymbol\endcsname}}}{\relax}%
    \coloredtext{\csname#2commentcolor\endcsname}{##1}%
  }%
  \expandafter\def\csname#2@ins\endcsname{\relax}
  \expandafter\renewcommand\csname#2@ins\endcsname[2][]{%
    \rule{0mm}{1ex}%
    \ifthenelse{\not\equal{\csname#2inssymbol\endcsname}{off}}{%
    \marginpar{\center\textcolor{\csname#2inscolor\endcsname}{%
               \csname#2inssymbol\endcsname}}}{\relax}%
    \coloredtext{\csname#2rmcolor\endcsname}{##1}%
    \ifthenelse{\equal{##1}{}}{\relax}{$\to$}%
    \coloredtext{\csname#2inscolor\endcsname}{##2}%
  }%
  \expandafter\def\csname#2@rm\endcsname{\relax}
  \expandafter\renewcommand\csname#2@rm\endcsname[2][]{%
    \rule{0mm}{1ex}%
    \ifthenelse{\not\equal{\csname#2rmsymbol\endcsname}{off}}{%
    \marginpar{\center\textcolor{\csname#2rmcolor\endcsname}{%
               \csname#2rmsymbol\endcsname}}}{\relax}%
    \coloredtext{\csname#2inscolor\endcsname}{##1}%
    \ifthenelse{\equal{##1}{}}{\relax}{$\ot$}%
    \coloredtext{\csname#2rmcolor\endcsname}{##2}%
  }%
  \expandafter\gdef\csname#2on\endcsname{%
    \cslet{#2par}{#2@par}%
    \cslet{#2inspar}{#2@inspar}%
    \cslet{#2rmpar}{#2@rmpar}%
    \cslet{#2ins}{#2@ins}%
    \cslet{#2rm}{#2@rm}%
    \cslet{#2com}{#2@com}%
  }%   
  \expandafter\gdef\csname#2off\endcsname{%
    \cslet{#2par}{skippar}%
    \cslet{#2inspar}{justpar}%
    \cslet{#2rmpar}{skippar}%
    \cslet{#2ins}{justins}%
    \cslet{#2rm}{justrm}%
    \cslet{#2com}{justrm}%
  }%   
  \csname#2on\endcsname
} 

%% Remark
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SET
%\def\st{\,\middle\vert\hspace{-1.5pt}\middle\vert\,}
\def\st{\;{\bm :}\;}
\def\set#1{\left\{#1\right\}}
%% SET
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% HYPERLINKS


\let\termtexthook=\relax
\let\termmarginhook=\relax
\let\seehook=\relax
\def\termmargin{no}

\def\termtexthook{\em}
\def\termmarginhook#1{\color{blue}\fbox{\parbox{\marginparwidth}{\raggedright#1}}}
\def\seehook#1{\color{gray}\underline{#1}}

\def\allterms{}

\newcommand{\term}[2][EMPTY]{%
  \ifthenelse{\equal{#1}{EMPTY}}%
    {\hypertarget{t:#2}{{\termtexthook{#2}}}%
      %\xdef\allterms{\allterms\ #2 \thepage,}%
      }%
    {\hypertarget{t:#1}{{\termtexthook{#2}}}%
      %\xdef\allterms{\allterms\ #1 \thepage,}
      }%
  \ifthenelse{\equal{\termmargin}{yes}}
    {\marginpar{\termmarginhook{#2}}}%
    {\relax}%
}
\renewcommand{\term}[2][EMPTY]{\emph{#2}}

\renewcommand{\see}[2][EMPTY]{%
  \hypersetup{linkcolor=blue}      
  \ifthenelse{\equal{#1}{EMPTY}}%
    {\hyperlink{t:#2}{{\seehook{#2}}}}%
    {\hyperlink{t:#1}{{\seehook{#2}}}}%
  \hypersetup{linkcolor=red}  
}  

%% HYPERLINKS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% EQUATION TAGS
\newcounter{subequation}[equation]
\makeatletter\@addtoreset{equation}{section}\makeatother
\def\defaulteqtag{\thesection.\arabic{equation}}
\def\defaultsubeqtag{\defaulteqtag.\alpha{subequation}}
\def\printeqlabel#1{\protect\makebox[0mm][l]{%
    \hspace{-3mm}\protect\raisebox{1em}{\tiny\color{red}#1}}}
\newcommand{\tageq}[2][empty]{%
   \ifthenelse{\equal{#1}{empty}}
     {%
      \stepcounter{equation}%
      %\tag{\defaulteqtag\printeqlabel{eq:#2}}%
      \tag{\defaulteqtag}%
     }
     {%
     %\tag*{#1\printeqlabel{eq:#2}}%
     \tag{#1}%
     }%
     \label{eq:#2}%
}
%% EQUATION TAGS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% THEOREMS etc
\def\empty{}
\xdef\listofclaims{}
\def\globallet#1#2{\global\let#1#2}
\def\epropsymbol{$\boxtimes$}
\def\eprop{ \rule{0.00mm}{3mm}\nolinebreak\hfill\epropsymbol}
\def\printlabel#1{\makebox[0mm][l]{%
    \hspace{-3mm}\raisebox{1em}{\tiny\color{red}#1}}}
\def\Label#1{\printlabel{#1}\label{#1}}
\newcommand{\NewTheorem}[3]{% {envname}{title}{countername}
  \newtheorem{#1nosave}[#3]{#2}
  \NewEnviron{#1}[1]
  {
    \xdef\lastclaim{##1}%
    \expandafter\xdef\csname##1countername\endcsname{the#3}
    \expandafter\xdef\csname##1envname\endcsname{#1nosave}
    \expandafter\globallet\csname##1content\endcsname=\BODY
    \xdef\listofclaims{\listofclaims,##1}
    \begin{#1nosave}\label{##1}%
      \expandafter\xdef\csname##1number\endcsname{\csname
        the#3\endcsname}
      % for draft
      %  \printlabel{##1}%
        \expandafter\ifx\csname r@##1.rep\endcsname\relax\else
          \hyperref[##1.rep]{\boldmath$\downarrow$}
        \fi          
        \BODY\eprop
    \end{#1nosave}
  }
}

\newif\ifclaimismissing
\claimismissingfalse

\newcommand{\repeatclaim}[1]{%
  \xdef\lastclaim{#1}%
   \expandafter\ifx\csname#1content\endcsname\relax
      {\mbox{\relax}\par\noindent\color{red}\bf Missing claim
      ``#1''.\par%
      \global\claimismissingtrue%
      }
   \else
     \global\claimismissingfalse%
     \begingroup%
     \expandafter\def\csname\csname#1countername\endcsname\endcsname{%
       \csname#1number\endcsname}
     \begin{\csname#1envname\endcsname}\label{#1.rep}
       % For draft
         %\printlabel{#1.rep}%
         \hyperref[#1]{\boldmath$\uparrow$} 
       \let\label=\skipthis
       \let\Label=\skipthis
       \let\marginpar=\skipthis
       \let\todo=\skipthis
       \csname#1content\endcsname
       \eprop
     \end{\csname#1envname\endcsname}
   \endgroup%
   \fi
}

\def\repeatallclaimsaux,#1;EndOfTheArgs{
  \foreach \claim in {#1}{
    \repeatclaim{\claim}
  }
}

\def\repeatallclaims{%
  \ifx\listofclaims\empty%
    \relax%
  \else%
    \expandafter\repeatallclaimsaux\listofclaims;EndOfTheArgs%
  \fi%
}
\newtheorem{Alphastatements}{XXX}
\def\theAlphastatements{\Alph{Alphastatements}}
\newtheorem{independent}{XXX}
\newtheorem{withinsection}{XXX}[section]
\newtheorem{withinsection1}{XXX}[section]

\NewTheorem{definition}{Definition}{withinsection}
\NewTheorem{proposition}{Proposition}{withinsection}
\NewTheorem{theorem}{Theorem}{withinsection}
\NewTheorem{corollary}{Corollary}{withinsection}
\NewTheorem{lemma}{Lemma}{withinsection}
\NewTheorem{tlemma}{Lemma}{withinsection1}
\NewTheorem{alphatheorem}{Theorem}{Alphastatements}
\NewTheorem{alphaconjecture}{Conjecture}{Alphastatements}
 
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}[conjecture]{Question}
\renewcommand{\theconjecture}{Q\arabic{conjecture}}

\def\eproofsymbol{$\boxtimes$}

\NewEnviron{Proof}[1][\lastclaim]{%
  \expandafter\ifx\csname#1content\endcsname\relax
     {\mbox{\relax}\par\color{red}\bf Skipping proof of ``#1''.%
      \nolinebreak\hfill\eproofsymbol\par}%
   \else
     \par\noindent\textit{Proof:} \BODY%
     \rule{0.00mm}{3mm}\nolinebreak\hfill\eproofsymbol\par
   \fi  
}

\def\eproof{\rule{0.00mm}{3mm}\nolinebreak\hfill\eproofsymbol\par}
%\newcommand{\proof}[1][]{\par\noindent\textit{Proof%
%    \ifthenelse{\equal{#1}{}}{:\ }{ (#1):\ }}%
%    }

\renewenvironment{proof}[1][missing]
{\medskip\par\noindent
  \ifthenelse{\equal{#1}{missing}}
  {\textit{Proof:} }
  {\textit{Proof}\textrm{(#1)}: }
}
{\rule{0.00mm}{3mm}\nolinebreak\hfill\eproofsymbol\par\medskip}
%% THEOREMS etc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% COMMUTATIVE DIAGRAMS
\tikzset{
  symbol/.style={
    draw=none,
    every to/.append style={
      edge node={node [sloped, allow upside down, auto=false]{$#1$}}}
  }
}
\NewEnviron{skipenv}{\relax}
\newenvironment{cd}[1][]
               {\begin{tikzcd}[ampersand replacement=\&,#1]}
               {\end{tikzcd}}

\newcommand{\cdon}{%
  \renewenvironment{cd}[1][]
                 {\begin{tikzcd}[ampersand replacement=\&,##1]}
                 {\end{tikzcd}}%
}

\newcommand{\cdoff}{%
  \renewenvironment{cd}[1][]
                 {\textcolor{red}{\text{Commutative diagram}}%
                  \begin{skipenv}%
                 }
                 {\end{skipenv}}%
}

%%% COMMUTATIVE DIAGRAMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatother

